Vertical shear instability in two-moment radiation-hydrodynamical simulations of irradiated protoplanetary disks I. Angular momentum transport and turbulent heating

We studied the linear and nonlinear evolution of the Vertical Shear Instability (VSI) in axisymmetric models of protoplanetary disks, focusing on the transport of angular momentum, the produced temperature perturbations, and the applicability of local stability conditions. We modeled the gas-dust mixture via high-resolution two-moment (M1) radiation-hydrodynamical simulations including stellar irradiation with frequency-dependent opacities. We found that, given sufficient depletion of small grains (with a dust-to-gas mass ratio of $10\%$ of our nominal value of $10^{-3}$ for $<0.25$ $\mu$m grains), the VSI can operate in surface disk layers while being inactive close to the midplane, resulting in a suppression of the VSI body modes. The VSI reduces the initial vertical shear in bands of approximately uniform specific angular momentum, whose formation is likely favored by the enforced axisymmetry. Similarities with Reynolds stresses and angular momentum distributions in 3D simulations suggest that the VSI-induced angular momentum mixing in the radial direction may be predominantly axisymmetric. The stability regions in our models are well explained by local stability criteria, while the employment of global criteria is still justifiable up to a few scale heights above the midplane, at least as long as VSI modes are radially optically thin. Turbulent heating produces only marginal temperature increases of at most $0.1\%$ and $0.01\%$ in the nominal and dust-depleted models, respectively, peaking at a few (approximately three) scale heights above the midplane. We conclude that it is unlikely that the VSI can, in general, lead to any significant temperature increase since that would either require it to efficiently operate in largely optically thick disk regions or to produce larger levels of turbulence than predicted by models of passive irradiated disks.

==> diskmodel.tex <==
 \section{Disk structure and stability}\label{S:DiskModel}
 
 \subsection{Initial condition} \label{S:InitialCondition}
 
The hydrostatic equilibrium conditions can
be obtained by setting all time derivatives to zero in Eqs. \eqref{Eq:RadHD}.
Additionally, we neglect viscous and radiative momentum exchange by setting $\mathbf{G}$ to zero. This
choice is justified since... \GREEN(order of magnitude)\BLACK
Thus, the $(r,\theta)$ components of the static momentum conservation equation are
\begin{equation}\label{Eq:Hydrostatic}
    \begin{split}
        \frac{\partial p_g}{\partial r} &=
        -\rho \frac{\partial \Phi}{\partial r}
        + \frac{\rho v_\phi^2}{r}  \\
        \frac{1}{r} \frac{\partial p_g}{\partial \theta}
        & = \frac{1}{\tan \theta}  \frac{\rho v_\phi^2}{r}\,.
    \end{split}
\end{equation}
The equilibrium configuration is obtained by
assuming a given vertically integrated density
distribution $\Sigma(r)$. The midplane gas
density is then computed in
terms of the local scale heigth
$H=\sqrt{(\mu u T_m/k_B)\, r^3/G M_s}$ as
$\rho(r,\theta=\pi/2)=\Sigma (r)/\sqrt{2\pi}H$, where $M_s$ is the star mass and $T_m$ is the
midplane temperature. This approximation holds
if the mass distribution is vertically Gaussian, which is true close to the midplane provided the temperature profile is vertically isothermal. 
This condition is in fact ferified close to 
the midplane, where most of the mass is located.
Once the midplane density is known, Eq.
\eqref{Eq:Hydrostatic} is integrated as detailed
in \cite{Flock2013} using the known temperature
distribution, and new $(\rho,v_\phi)$ values
are computed in the entire domain. The
Rad-HD equations are then integrated assuming the new configuration to be static \GREEN(rewrite)\BLACK,
and a new temperature distribution  is obtained. The whole process is repeated until convergence
of the temperature and density distributions \GREEN(convergence criterion)\BLACK.

\GREEN Boundary conds.  \BLACK

